Counterfactual Causality from First Principles?

In this position paper we discuss three main shortcomings of existing approaches to counterfactual causality from the computer science perspective, and sketch lines of work to try and overcome these issues: (1) causality definitions should be driven by a set of precisely specified requirements rather than specific examples; (2) causality frameworks should support system dynamics; (3) causality analysis should have a well-understood behavior in presence of abstraction.

==> eptcsdata.tex <==
\providecommand{\firstpage}{47}
\providecommand{\publicationstatus}{A. Groce and S. Leue: 2nd International Workshop on Causal Reasoning\\ for Embedded and safety-critical Systems Technologies (CREST'17)\\
EPTCS 259, 2017, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.259.5}{10.4204/EPTCS.259.5}}

